MuMuQA: Multimedia Multi-Hop News Question Answering via Cross-Media Knowledge Extraction and Grounding

Recently, there has been an increasing interest in building question answering (QA) models that reason across multiple modalities, such as text and images. However, QA using images is often limited to just picking the answer from a pre-defined set of options. In addition, images in the real world, especially in news, have objects that are co-referential to the text, with complementary information from both modalities. In this paper, we present a new QA evaluation benchmark with 1,384 questions over news articles that require cross-media grounding of objects in images onto text. Specifically, the task involves multi-hop questions that require reasoning over image-caption pairs to identify the grounded visual object being referred to and then predicting a span from the news body text to answer the question. In addition, we introduce a novel multimedia data augmentation framework, based on cross-media knowledge extraction and synthetic question-answer generation, to automatically augment data that can provide weak supervision for this task. We evaluate both pipeline-based and end-to-end pretraining-based multimedia QA models on our benchmark, and show that they achieve promising performance, while considerably lagging behind human performance hence leaving large room for future work on this challenging new task.

==> bak/1_introduction_bak.tex <==
\section{Introduction}

\begin{figure*}[ht]
     \begin{subfigure}[b]{0.48\textwidth}       
     \includegraphics[scale=0.36]{img/ex_1.png}       \caption{}
       \label{fig:mmqa_example_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}       
     \includegraphics[scale=0.22]{img/ex_4.png}       \caption{}
       \label{fig:mmqa_example_2}
     \end{subfigure}
     \caption{Two examples from our evaluation benchmark with the question-answer pairs and their corresponding news articles. The bridge item, which needs to be grounded from image onto text, is shown in red and the final answer is marked in green in the news body text. %\heng{the wording of the question in (a) is still a bit awkward. maybe change it to 'What party does the person with the blue tie in the image belong to?'}
     }
     \label{fig:walkthrough_example}
%\vspace{-0.5cm} 
\end{figure*}


%Question Answering (QA) requires a model to respond to a specified question by leveraging context provided in the form of  images, text or structured data such as graphs and tables \jc{While leveraging context beyond text is our goal, `QA' usually refers to text-only QA. So ``QA requires model to leverage context in the form of image'' sounds a bit unnatural to me.}. 
To answer questions, humans seamlessly combine context provided in the form of images, text, background knowledge or structured data such as graphs and tables. Availability of a similarly capable question answering (QA) model could increase information accessibility and allow 
%enabling the blind to 
quick understanding of news or scientific articles, where the main narrative is enriched by images, charts and graphs with captions.

%context, i.e., images, charts and graphs with captions. %QA also enables interaction with news in a hands-free manner, e.g., when driving a car.  
%
However, most QA research to date focuses on extracting information from a single data modality, such as text (TextQA) \cite{rajpurkar2016squad, kwiatkowski2019natural}, images (VQA) \cite{antol2015vqa, goyal2017making} or videos (VideoQA) \cite{yang2003videoqa}. Only recently, there have been initial attempts to combine information from multiple modalities \cite{kembhavi2017you,lei2018tvqa}, which often use %however \jc{'however' implies something negative for multiple choice questions, but they are not mentioned} have 
questions in a multiple-choice setting. However, multiple choice questions in VQA have been shown to have explicit bias \cite{kazemi2017show, manjunatha2019explicit}, which can be taken advantage of by using question understanding or answer option analysis. %\heng{add the second limitation: lack of knowledge grounding which is required in the reaoning process for many multi-hop questions. }

To address this concern, more recently, \citet{talmor2021multimodalqa} introduce an extractive multi-hop QA dataset that involves reasoning across tables, text and images. However, each image is associated with a Wikipedia entity and thus, reasoning over images essentially boils down to ranking the images based on the question and using the entities corresponding to the top-ranked images. 
%In constrast, questions about images in real-life typically  require identifying which object in the image is being referred to, so as to leverage background knowledge for answering the question.\lifu{The description of this previous dataset cannot clearly show the unique challenges of \taskname{}. We should emphasize: (1) previous dataset does not require cross-media reasoning between images and the context (2) most of them do not require multi-hop reasoning}\avi{Agree with Lifu.}
In contrast, questions about images in real life require cross-media reasoning between images and text. %, so as to leverage background knowledge for answering the question. %\as{maybe drop `so as to leverage background knowledge for answering the question?; `background knowledge' may imply use of knowledge basis?} 
Current multimodal benchmarks cannot be used to solve this as they do not require to ground images onto text when answering questions about images.

To bridge this gap, we introduce a new benchmark QA evaluation task called `Multi-media Multi-hop Question Answering' (\taskname{}) %over news articles 
along with a corresponding dataset of news articles. To succeed in this new \taskname{} 
%\avi{I replaced MuMuQA with this global name. Do you like this font or the original? Fine either way but use the global name it's much easier to use everywhere.} 
task, methods need to excel at both identifying objects being referred to in the question and leveraging news body text to answer the question. Specifically, the task is formulated as multi-hop extractive QA where
questions focus on objects grounded in  image-caption pairs. To enforce multi-hop reasoning, we ask information-seeking questions about objects in the image by referring to them via their visual attributes. The requirement for grounding between image and text along with multi-hop reasoning makes \taskname{} much more challenging than the tasks which are commonly explored in the QA community so far.

Figure~\ref{fig:walkthrough_example} illustrates the task and the data. % \jc{task data sounds weird}.
Answering the question in Figure~\ref{fig:mmqa_example_1} requires first identifying that ``the person with the blue tie'' is on the right in the image, which needs to be grounded to ``Benjamin Netanyahu'' (in \textcolor{red}{red}) in the caption. Subsequently the news body text is needed to  extract the answer. Grounding between image-caption pairs along with textual understanding and coreference resolution is hence crucial.
%\lifu{here you need to explain a little bit of the example, and use the example to illustrate the challenges of MuMuQA, e.g., multihop reasoning, grounding with visual attributes}
Note that %it can be seen that 
the question cannot be  answered by a text-only model, % which picks the name of the party, 
since the text mentions two parties  (\textcolor{ForestGreen}{green} and \textcolor{YellowOrange}{yellow} highlight) % Dandelion %\avi{this yellow is unreadable.} 
that correspond to the two people in the image-caption pair (names in \textcolor{red}{red} and \textcolor{brown}{brown}).
%Grounding between image-caption pairs along with textual understanding and coreference resolution is crucial.


To study \taskname{}, we release an evaluation set with 263 development and 1,121 test examples. Annotators were asked to identify objects grounded in image-caption pairs and come up with questions about them which can be answered by the news body text.
%\lifu{Briefly describe how the examples are created} 
Given the high cost of annotating such examples, we use human-curated examples only as the evaluation set and develop a novel multimodal data augmentation approach %\heng{need to explain what the approach is, give a short summary on how it works} 
to automatically generate silver-standard training data for this task, which can then be used to train or fine-tune state-of-the-art (SOTA) vision-language models \cite{tan2019lxmert, li2020oscar}. Specifically, we generate silver training data by leveraging multimedia information extraction (IE), visual scene understanding and language generation. In short, we first run a multimedia IE system \cite{li2020gaia} to capture the entities that are grounded in image-caption pairs, such as ``Benjamin Netanyahu''. Next, we apply a question generation approach \cite{shakeri2020end} to automatically generate questions from the news body text, that are conditioned on one of the grounded entities, such as ``What party does Benjamin Netanyahu belong to?''. Then, we use a visual attribute recognition model \cite{lin2019improving} to edit these questions to refer to the grounded entity by its visual attributes, such as replacing ``Benjamin Netanyahu'' with ``the person with the blue tie'' in the question. Finally, we filter out questions that are answerable by a single-hop text-only QA model \cite{chakravarti2020towards}. %\heng{maybe walk through these steps using examples.}\manling{To avoid repeating sec 4.1, I continue using example of Figure 1, instead of Figure 3. Please check whether it is okay. } 
This pipeline automatically generates %weakly supervised 
training data for our task.
%\heng{you still need to briefly describe how the pipeline QA and end-to-end QA work}

%\heng{maybe give a table to summarize the comparison among various benchmarks, explain the criteria/principles in your design: 1. multi-media information fusion; 2. multi-hop reasoning. and how you achieve these goals}


We evaluate both text-only QA and multimedia QA models on our \taskname{} benchmark. Particularly, we explore both pipeline-based and end-to-end multimedia QA approaches. The pipeline-based model first decomposes the task into image-question and text-question. Then, it uses a SOTA multimedia IE model~\cite{li2020gaia} for visual entity grounding and attribute matching to answer the image-question and uses a single-hop text QA model~\cite{chakravarti2020towards} to extract the final answer.
%\haoyang{we may need some citations, not sure which one to cite}
For the end-to-end multimedia QA system, we directly finetune a SOTA visual-language pretrained model~\cite{li2020oscar} using auto-generated silver-standard training data.
%\mbc{we need another para after this for the models on our task and results, right? just like the last line in the abstract? otherwise can be risky/confusing to end} \heng{agree with this}

%\heng{need to emphasize the novelty of QA method, the multimedia knowledge representation is new? use multimedia IE is new? add a bullet below}


The contributions of this work are as follows:
\begin{itemize}
    \item We release a new extractive QA evaluation benchmark, \taskname{}. It is based on multi-hop reasoning and cross-media grounding of information present in news articles. 
   To the best of our knowledge, our work is the first to explore using information grounded in the image in an extractive QA setting (see Section~\ref{sec:task} and Section~\ref{sec:data}).
   % To the best of our knowledge, our work is the first to explore cross-media information grounding in a multi-hop extractive QA setting (see Section~\ref{sec:task}).
    \item To automatically generate silver-standard training data for this task, we introduce a novel pipeline that incorporates cross-media knowledge extraction, visual understanding and synthetic question generation (Section~\ref{sec:syn_data}). %  to automatically generate weakly-supervised training data and use it to fine-tune current SOTA multi-media models to our task.
    \item We measure the impact of images in our benchmark by evaluating competitive text-only QA models on our task, and
    demonstrate the benefit of using multimedia information (see Section~\ref{sec:QAModels}).
    %demonstrate the inadequacy of information from using just the body text (see Section~\ref{sec:QAModels}).
\end{itemize}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Below this is all commented out parts of the INTRO



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse


%Question Answering (QA) is a task of automatically answering questions posed by humans in natural language.  Typically, the answer is expected to come from some background information. \heng{So one big confusion is the term 'background information'/'background knowledge'. It took me a while to figure out you actually mean 'extract background information from body text'. It will be good to use a different term or define/clarify it early} Information in the real world appears in multiple formats, such as images, text and also structured data like graphs and tables. An example of a domain with information grounded across formats is news articles, which typically contain images describing the news event, their corresponding captions and finally the textual context of the news article. Thus, QA is particularly important and useful in such domains, for any user seeking a rich, rapid and deep understanding of an emergent situation.

However, most QA research till date  focuses on extracting information from a single modality, such as text (TextQA) \cite{rajpurkar2016squad, kwiatkowski2019natural}, visuals (VQA) \cite{antol2015vqa, goyal2017making} or videos (VideoQA) \cite{yang2003videoqa}. Only recently, there have been first attempts to combine information from multiple modalities, e.g. videos and captions \cite{lei2018tvqa} or images and descriptions in textbooks \cite{kembhavi2017you}. However, these first methods are  restricted in two ways: 1) they consider the discriminative multiple choice QA setting, i.e., picking the correct answer from a given set of options; and 2) they often don't require careful multi-hop reasoning between narrative and context. %don't require any external background knowledge to answer questions. 

Both restrictions are severe. First, questions in a real-world setting \cite{kwiatkowski2019natural,clark2020tydi} %I added 2 citations to NQ and TyDI: TyDi is missing you can add that.} 
are often not multiple-choice but rather `extractive', i.e.,  the answer corresponds to some part of the narrative. Second, finding the correct part of the narrative often requires to combine information from both context and narrative. %, by combining information that might be presented in multiple data modalities in a complimentary way. 
To see this consider the news articles shown in Fig.~\ref{fig:walkthrough_example} and their context given in the form of an image-caption pair. %Fig.~\ref{fig:mmqa_example_1} shows an example news article along with a corresponding image-caption pair and its annotated question-answer pair.
Answering the specified question requires 1) to find the right part of the text via 2) \textit{multi-hop} reasoning between context and narrative. E.g., methods can use the context (image-caption pair) to identify the \textit{person with the blue tie} as Benjamin Netanyahu (in \textcolor{RubineRed}{red}) \avi{Some reviewers \textit{may} complain that you shouldn't use colors for color-blind readers.}and then use the news article %text as the background knowledge 
to extract the answer. Note that %it can be seen that 
the question cannot be  answered by a text-only model, % which picks the name of the party, 
since the text mentions two parties  (\textcolor{ForestGreen}{green} and \textcolor{YellowOrange}{yellow} highlight) % Dandelion %\avi{this yellow is unreadable.} 
that correspond to the two people in the image-caption pair (names in \textcolor{red}{red} and \textcolor{brown}{brown}). %Hence, the text alone would be incomplete to answer the question as the image provides essential complementary information, that further needs to be grounded with the caption. 
%Fig.~\ref{fig:mmqa_example_2} provides another example. Here, the group needs to be grounded as \textit{Belt and Road Forum}, with the body text mentioning that \textit{India} skipped the summit. Essentially, our QA task involves image understanding, cross-media %\heng{make the terms consistent between 'modal' and 'media'. maybe just call everything as cross-media or multi-media} 
Grounding between image-caption pairs along with textual understanding and coreference resolution is crucial. %\heng{use 'coreference resolution' instead of 'co-reference' throughout the paper.}


Both the extractive setting and the multi-hop reasoning make the real-world QA setting  much more challenging than the tasks which are commonly explored in the QA community so far. %\revanth{Point out limitations of multi-choice settings here: answering by elimination} \avi{I think the motivation needs to be stronger. Let's brainstorm together on what the issues are with these datasets. I'd say the major issue is that we don't have labeled QA pairs that tend to require all modes which is required for reason 1, 2 \& 3 ?}

To bridge this gap we introduce the new benchmark QA evaluation task `Multi-media Question Answering' (\taskname{}) and a corresponding dataset. To succeed in this new \taskname{} task, methods need to excel at both of the aforementioned limitations. %explores the interaction between knowledge elements presented in different data modalities in news articles. 
Specifically, the \taskname{} task is formulated as  extractive QA  %that requires answers to be extracted from the news article, for 
where 
questions focus on objects grounded in the image-caption pairs. To enforce multi-hop reasoning, we ask information-seeking questions about objects in the image by referring to them via their visual attributes.  \revanth{Point out here that Multimedia QA does not require any grounding}


% \heng{try to use 'approach/framework' instead of 'system' whenever possible}

%\heng{the walk through example needs to be changed to a more informative one}

%Figure \ref{fig:mmqa_example} shows an example news article from our task. For this news article, Figure \ref{fig:mmqa_example_questions} shows a question from our \taskname{} task, that involves multimedia reasoning, compared with existing QA benchmarks that involve reasoning over a single modality, such as TextQA or VQA. 
Fig.~\ref{fig:walkthrough_example} illustrates   our \taskname{} task data. Fig.~\ref{fig:mmqa_example_1} shows an example news article along with a corresponding image-caption pair and its annotated question-answer pair.
Note, answering the question requires \textit{multi-hop} reasoning across modalities: the framework first needs to use the image-caption pair to identify the \textit{person with the blue tie} as Benjamin Netanyahu (in \textcolor{RubineRed}{red}) \avi{Some reviewers \textit{may} complain that you shouldn't use colors for color-blind readers.}and then use the news article %text as the background knowledge 
to extract the answer. Importantly, %it can be seen that 
the question cannot be directly answered by a text-only model which picks the name of the party, since the text mentions two parties  (in \textcolor{ForestGreen}{green} and \textcolor{YellowOrange}{yellow}) % Dandelion %\avi{this yellow is unreadable.} 
that correspond to the two people in the image-caption pair (in \textcolor{red}{red} and \textcolor{brown}{brown}). Hence, the text alone would be incomplete to answer the question as the image provides essential complementary information, that further needs to be grounded with the caption. 
Fig.~\ref{fig:mmqa_example_2} provides another example. Here, the group needs to be grounded as \textit{Belt and Road Forum}, with the body text mentioning that \textit{India} skipped the summit. Essentially, our QA task involves image understanding, cross-media %\heng{make the terms consistent between 'modal' and 'media'. maybe just call everything as cross-media or multi-media} 
grounding between image caption pairs along with textual understanding and coreference resolution. %\heng{use 'coreference resolution' instead of 'co-reference' throughout the paper.}

\heng{Why do we need a new data set and a new QA framework? Point out the limitations of multi-choice settings: 1. it's not realistic setting; 2. some choices from crowd sourcing tend to be too artificial; 3. allow semantic matching system to cheat} \avi{Okay so Heng already pointed this out here ( I didn't see this when I wrote similar comment in the prev page) whereas I think we should motivate even before we introduce our dataset. But we agree that the motivation needs to be strong ASAP to the reader before he/she starts figuring out issues in their heads.}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%COMMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Old Introduction}


% \heng{multimedia reasoning based QA, experiments: separate How/Why questions from other Ws}


% \heng{main contributions: 1. a new multimedia QA benchmark; 2. use multimedia kb common space for question generation; 3. add kb matching for QA; 4. questions involve multimedia and multihop, focus on information needs, more realistic}

% %qa: realistic questions derived from captions, multimedia, structured knowledge base, first event


% QA: informativeness, cross-media, detectable

% input:
% image + surrounding texts without caption

% qa automatically generated from caption IE + human curation

% contributions:
% 1. a new task, benchmark, data annotations
% 2. use multimedia common space
% 3. use IE
% 4. how to do reasoning?
% 5. how to handle cross-sentence information?


% to-do: check results to see if IE results look ok:

% image,
% caption + IE
% contextual sentences in surrounding text that include the same events as in captions



% Give a reference document or a collection of reference documents, Question Answering (QA) is a task to automatically answer questions posed by humans in a natural language. The QA task is particularly important and useful for any user seeking a rich, rapid and deep understanding of an emergent situation. However, state-of-the-art QA tasks and techniques cannot meet this requirement. In this paper we aim to advance state-of-the-art by addressing two limitations as follows. 

% Current QA research methods target a single modality, such as text~\cite{voorhees1999trec}, images~\cite{antol2015vqa} or videos~\cite{yang2003videoqa}. However, real-time information about most emergent situations is often presented in multiple data modalities in a complementary way. The sheer volume and diversity of such information makes the QA task an immensely challenging one. 
% Moreover, most of the existing QA tasks focus on entities and relations in a single reference document. Very little work has been done on complex events in news events which require deep understanding of background knowledge. 


% For example, after the U.S. killed top Iranian military commander Qasem Soleimani, we can expect many consequent events happening. In an interview video as shown in Figure~\ref{img:vqa_example}, we may want to know who is the interviewee (Iran's foreign minister Javad Zarif). In an image about protest, we may want to know where the protest is taking place (Tehran).

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=1.0\linewidth]{img/vqa_example.pdf}
% \caption{Example input of multimedia question answering. }
% \label{img:vqa_example}
% \end{figure}


% Simple baseline methods that only use question understanding~\cite{kazemi2017show} or answer option sentiment analysis~\cite{manjunatha2019explicit} have been proven surprisingly well on data sets such as VQA~\cite{antol2015vqa} and VQA2.0~\cite{goyal2017making}. But they are unlikely to provide good answers for understanding complex events. We propose a new multimedia news question answering benchmark where we focus on questions that require background knowledge acquisition and reasoning, and informative answers that can be verified from multiple data modalities. The input is an image or a video, along with a set of background text documents. We derive questions semi-automatically from the captions of the target images and videos. We propose a novel method to extract background knowledge from the related text documents.

% \heng{add detailed methods}

% In addition, real events are hierarchical and probabilistic. Understanding them requires knowledge in the form of a repository of abstracted event schemas (complex event templates), understanding the progress of time, using background knowledge, and performing global inference. 

% For example, in the history, when similar attack events happening, usually the leaders of both countries will give speech, some  protests will occur, and more attack events may happen.

% A schema is illustrated in Figure XXX.

% \heng{consider to re-use the schema figure in the proposal, and the event examples need to be replaced.}

% We propose a novel framework to actively acquire and tightly integrate 
% knowledge from a massive amount of multi-media multi-lingual news, encyclopedia resources and event 
% ontologies for probabilistic schema induction, and enrich our acquired schemas with novel temporal attribute discovery. 
% Then we develop a novel schema-guided event reasoning and 
% prediction framework that can extract, verify and infer the answers from the target images and videos.



% history repeats itself...

% We propose 


% Once we have acquired a large-scale %bank of 
% schema repository in TA1, we can view it as providing a scaffolding that we can instantiate with incoming data to construct a temporal event knowledge base. 
% %We may also be aware of additional, background information (e.g., past similar events in the same location, etc.) that we would like to incorporate to further improve our prediction abilities. 
% %We propose to incorporate additional background information (e.g., past similar events in the same location) to further improve our prediction abilities.
% We propose a novel reasoning framework that is guided by schemas, background knowledge (e.g., past events that are similar and in the same location) and temporal constraints, and multi-media information. Table~\ref{tab:schemamatchingexample} provides some motivating examples.
% %to motivate our use of event schema and background knowledge, temporal reasoning, abstraction, and multi-media information, all working together via our reasoning framework.
% Our framework will use these to improve our event extraction, temporal and causal tracking, subevent relation extraction and prediction abilities. The framework will 
% %is informed by a collection of data-driven models used to 
% induce abstractions for long-term event forecasting, and it uses its prediction results as feedback to refine the schemas in TA1 and further improve extraction, tracking and prediction. 










% use multimedia structured representation... schema induction


% Input: given an image and surrounding text (not captions), try to answer questions related to events

% novel ideas:

% problems: question only, sentiment only
% a more realistic task

% Setting 1:
% Input: news summary from the beginning of the video  &  news video
% Output: current event

% Setting 2:
% Input: background news  &  news video
% Output: current event

% Dataset preprocessing:
% Video ASR
% Image OCR


% (1) explore news domain
% (2) discover schema from old data, apply to the new images/videos (KAIROS TA2.1)
% (3) multi-hop query (event graph / image graph)

% important to understand events; multimedia important; intel analysis typical questions often involve images


% Problems on existing data sets:

% 1. lack of scenarios related to newsworthy complex events; understanding events is critical to understand the world
% 2. for images in news, we can automatically create q anda , thanks to information redundancy. 
% 3. 

% We have created a new benchmark that includes XXX question and answer pairs, showed multiple methods


% The current VQA data sets are very artificial: if we only use question sentence we can get good scores; if we only pick answer with positive sentiment, we get good scores etc.

% I'm thinking that since now in VOA news data set, for each image we know which text sentence is the most relevant one (maybe caption or other sentence), then we can run our multimedia event extraction, and convert the statement text sentence to question sentence automatically, by replacing an argument with a 5W1H question slot. Some examples are at:



